Shopping with a Platform AI Assistant: Who Adopts, When in the Journey, and What For

This paper provides some of the first large-scale descriptive evidence on how consumers adopt and use platform-embedded shopping AI in e-commerce. Using data on 31 million users of Ctrip, China's largest online travel platform, we study "Wendao," an LLM-based AI assistant integrated into the platform. We document three empirical regularities. First, adoption is highest among older consumers, female users, and highly engaged existing users, reversing the younger, male-dominated profile commonly documented for general-purpose AI tools. Second, AI chat appears in the same broad phase of the purchase journey as traditional search and well before order placement; among journeys containing both chat and search, the most common pattern is interleaving, with users moving back and forth between the two modalities. Third, consumers disproportionately use the assistant for exploratory, hard-to-keyword tasks: attraction queries account for 42% of observed chat requests, and chat intent varies systematically with both the timing of chat relative to search and the category of products later purchased within the same journey. These findings suggest that embedded shopping AI functions less as a substitute for conventional search than as a complementary interface for exploratory product discovery in e-commerce.

==> Results_New/When/order_adj_12h/table_chat_sequence_session_level.tex <==
\begin{table}[htbp!]
\centering
\caption{Chat-First vs.\ Chat-After-Search sessions ($N = 206,245$)}
\label{tab:chat_sequence_session}
\small
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
 & Chat-First & Chat-Between-Search & Chat-After-Search & Chat-Only \\
\midrule
\multicolumn{5}{l}{\textit{\textbf{Panel A: Prevalence}}} \\
Share of sessions & 21,911 (10.624\%) & 24,851 (12.049\%) & 20,975 (10.17\%) & 138,508 (67.157\%) \\
\addlinespace[0.35em]
\multicolumn{5}{l}{\textit{\textbf{Panel B: Session characteristics}}} \\
Mean session length (hours) & 0.787 & 1.192 & 0.781 & 0.422 \\
Mean chat sessions & 1.278 & 1.426 & 1.286 & 1.358 \\
Mean hotel searches & 11.33 & 35.772 & 11.245 & 0 \\
Mean clicks & 5.12 & 14.582 & 4.821 & 0 \\
Mean orders & 0.017 & 0.064 & 0.016 & 0.006 \\
Conversion rate (\%) & 1.123 & 1.887 & 1.073 & 0.39 \\
\addlinespace[0.35em]
\multicolumn{5}{l}{\textit{\textbf{Panel C: Chat intent distribution (\%)}}} \\
Attraction & 38.62 & 37.258 & 43.252 & 43.442 \\
Hotel & 33.232 & 43.123 & 29.943 & 8.78 \\
Travel Planning & 6.369 & 3.282 & 4.428 & 8.641 \\
Customer Service & 4.117 & 3.076 & 4.057 & 6.257 \\
Flight & 0.575 & 0.183 & 0.497 & 2.491 \\
Other Transportation & 4.213 & 3.46 & 4.647 & 10.378 \\
Other & 12.874 & 9.616 & 13.176 & 20.012 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\item \textit{Notes}: This table compares four groups of login sessions containing at least one AI chat. The first three groups additionally contain at least one hotel search within the session: \textit{Chat-First} sessions have all chat events before all search events; \textit{Chat-After-Search} have all chat events after all search events; \textit{Chat-Between-Search} have interleaved events. \textit{Chat-Only} sessions contain chat but no hotel search. Panel~A reports the number and share of sessions in each group. Panel~B reports session-level characteristics; differences across the three chat+search groups are all significant at the 0.1\% level (Kruskal--Wallis / chi-squared). Panel~C reports chat intent shares (summing to 100\% per column). Intent differs significantly across the three chat+search groups ($\chi^2 = 1705$, $p < 0.001$). $N = 206,245$ sessions.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Results_New/When/order_adj_8h/table_chat_sequence_session_level.tex <==
\begin{table}[htbp!]
\centering
\caption{Chat-First vs.\ Chat-After-Search sessions ($N = 206,245$)}
\label{tab:chat_sequence_session}
\small
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
 & Chat-First & Chat-Between-Search & Chat-After-Search & Chat-Only \\
\midrule
\multicolumn{5}{l}{\textit{\textbf{Panel A: Prevalence}}} \\
Share of sessions & 21,911 (10.624\%) & 24,851 (12.049\%) & 20,975 (10.17\%) & 138,508 (67.157\%) \\
\addlinespace[0.35em]
\multicolumn{5}{l}{\textit{\textbf{Panel B: Session characteristics}}} \\
Mean session length (hours) & 0.787 & 1.192 & 0.781 & 0.422 \\
Mean chat sessions & 1.278 & 1.426 & 1.286 & 1.358 \\
Mean hotel searches & 11.33 & 35.772 & 11.245 & 0 \\
Mean clicks & 5.12 & 14.582 & 4.821 & 0 \\
Mean orders & 0.017 & 0.064 & 0.016 & 0.006 \\
Conversion rate (\%) & 1.123 & 1.887 & 1.073 & 0.39 \\
\addlinespace[0.35em]
\multicolumn{5}{l}{\textit{\textbf{Panel C: Chat intent distribution (\%)}}} \\
Attraction & 38.62 & 37.258 & 43.252 & 43.442 \\
Hotel & 33.232 & 43.123 & 29.943 & 8.78 \\
Travel Planning & 6.369 & 3.282 & 4.428 & 8.641 \\
Customer Service & 4.117 & 3.076 & 4.057 & 6.257 \\
Flight & 0.575 & 0.183 & 0.497 & 2.491 \\
Other Transportation & 4.213 & 3.46 & 4.647 & 10.378 \\
Other & 12.874 & 9.616 & 13.176 & 20.012 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\item \textit{Notes}: This table compares four groups of login sessions containing at least one AI chat. The first three groups additionally contain at least one hotel search within the session: \textit{Chat-First} sessions have all chat events before all search events; \textit{Chat-After-Search} have all chat events after all search events; \textit{Chat-Between-Search} have interleaved events. \textit{Chat-Only} sessions contain chat but no hotel search. Panel~A reports the number and share of sessions in each group. Panel~B reports session-level characteristics; differences across the three chat+search groups are all significant at the 0.1\% level (Kruskal--Wallis / chi-squared). Panel~C reports chat intent shares (summing to 100\% per column). Intent differs significantly across the three chat+search groups ($\chi^2 = 1705$, $p < 0.001$). $N = 206,245$ sessions.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Results_New/When/table_chat_sequence.tex <==
\begin{table}[htbp!]
\centering
\caption{Journey Characteristics by Relative Timing of Chat and Search}
\label{tab:chat_sequence}
\footnotesize
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
 & Chat-First & Chat-Between-Search & Chat-After-Search & Chat-Only \\
\midrule
\multicolumn{5}{l}{\textit{\textbf{Panel A: Prevalence}}} \\
Share of journeys (\%) & 15.076 & 30.916 & 12.411 & 41.596 \\
%Number of journeys & 29,013 (15.076\%) & 59,496 (30.916\%) & 23,884 (12.411\%) & 80,048 (41.596\%) \\
\addlinespace[0.35em]
\multicolumn{5}{l}{\textit{\textbf{Panel B: Journey characteristics}}} \\
Median journey length (hours) & 51.809 & 94.837 & 51.97 & 18.405 \\
Mean login sessions & 11.313 & 28.625 & 10.538 & 5.582 \\
Mean chat sessions & 1.377 & 1.566 & 1.358 & 1.411 \\
Mean hotel searches & 24.365 & 150.029 & 21.433 & 0 \\
Mean clicks & 11.504 & 68.371 & 9.532 & 0 \\
Mean orders & 0.562 & 0.666 & 0.463 & 0.223 \\
Conversion rate (\%) & 39.382 & 43.166 & 31.13 & 18.04 \\
\addlinespace[0.35em]
\multicolumn{5}{l}{\textit{\textbf{Panel C: Chat intent distribution (\%)}}} \\
Attraction & 44.21 & 41.881 & 48.481 & 39.873 \\
Hotel & 17.927 & 30.388 & 17.681 & 7.062 \\
Travel Planning & 9.837 & 6.075 & 5.39 & 8.031 \\
Customer Service & 4.871 & 3.763 & 5.541 & 6.93 \\
Flight & 1.369 & 0.589 & 0.919 & 3.243 \\
Other Transportation & 6.233 & 4.87 & 5.615 & 12.692 \\
Other & 15.552 & 12.434 & 16.373 & 22.169 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\item \textit{Notes}: This table compares four groups of journeys containing at least one AI chat session. The first three groups additionally contain at least one hotel search: \textit{Chat-First} journeys have all chat events before all search events; \textit{Chat-After-Search} have all chat events after all search events; \textit{Chat-Between-Search} have interleaved chat and search events. \textit{Chat-Only} journeys contain chat but no hotel search. Panel~A reports the share and number of journeys in each group. Panel~B reports journey-level characteristics; differences across the three chat+search groups are all significant at the 0.1\% level (Kruskal--Wallis tests for continuous variables, chi-squared for conversion rate). Panel~C reports the distribution of chat intent categories within each group; intent shares sum to 100\% within each column (up to rounding). The intent distribution differs significantly across the three chat+search groups ($\chi^2 = 4{,}405.7$, $p < 0.001$).
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Results_New/When/table_chat_sequence_session_level.tex <==
\begin{table}[htbp!]
\centering
\caption{Session Characteristics by Relative Timing of Chat and Search}
\label{tab:chat_sequence_session}
\footnotesize
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
 & Chat-First & Chat-Between-Search & Chat-After-Search & Chat-Only \\
\midrule
\multicolumn{5}{l}{\textit{\textbf{Panel A: Prevalence}}} \\
Share of sessions (\%) & 10.624 & 12.049 & 10.170 & 67.157 \\
\addlinespace[0.35em]
\multicolumn{5}{l}{\textit{\textbf{Panel B: Session characteristics}}} \\
Mean session length (hours) & 0.787 & 1.192 & 0.781 & 0.422 \\
Mean chat sessions & 1.278 & 1.426 & 1.286 & 1.358 \\
Mean hotel searches & 11.330 & 35.772 & 11.245 & 0.000 \\
Mean clicks & 5.120 & 14.582 & 4.821 & 0.000 \\
Mean orders & 0.017 & 0.064 & 0.016 & 0.006 \\
Conversion rate (\%) & 1.123 & 1.887 & 1.073 & 0.390 \\
\addlinespace[0.35em]
\multicolumn{5}{l}{\textit{\textbf{Panel C: Chat intent distribution (\%)}}} \\
Attraction & 38.620 & 37.258 & 43.252 & 43.442 \\
Hotel & 33.232 & 43.123 & 29.943 & 8.780 \\
Travel Planning & 6.369 & 3.282 & 4.428 & 8.641 \\
Customer Service & 4.117 & 3.076 & 4.057 & 6.257 \\
Flight & 0.575 & 0.183 & 0.497 & 2.491 \\
Other Transportation & 4.213 & 3.460 & 4.647 & 10.378 \\
Other & 12.874 & 9.616 & 13.176 & 20.012 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\item \textit{Notes}: This table compares four groups of login sessions containing at least one AI chat. The first three groups additionally contain at least one hotel search within the session: \textit{Chat-First} sessions have all chat events before all search events; \textit{Chat-After-Search} have all chat events after all search events; \textit{Chat-Between-Search} have interleaved events. \textit{Chat-Only} sessions contain chat but no hotel search. Panel~A reports the share of sessions in each group. Panel~B reports session-level characteristics; differences across the three chat+search groups are all significant at the 0.1\% level (Kruskal--Wallis tests for continuous variables, chi-squared for conversion rate). Panel~C reports the distribution of chat intent categories within each group; intent shares sum to 100\% within each column (up to rounding). The intent distribution differs significantly across the three chat+search groups ($\chi^2 = 1{,}705$, $p < 0.001$). The sample consists of $N = 206{,}245$ sessions.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> Results_New/When/time_only_48h/table_chat_sequence_session_level.tex <==
\begin{table}[htbp!]
\centering
\caption{Chat-First vs.\ Chat-After-Search sessions ($N = 206,245$)}
\label{tab:chat_sequence_session}
\small
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
 & Chat-First & Chat-Between-Search & Chat-After-Search & Chat-Only \\
\midrule
\multicolumn{5}{l}{\textit{\textbf{Panel A: Prevalence}}} \\
Share of sessions & 21,911 (10.624\%) & 24,851 (12.049\%) & 20,975 (10.17\%) & 138,508 (67.157\%) \\
\addlinespace[0.35em]
\multicolumn{5}{l}{\textit{\textbf{Panel B: Session characteristics}}} \\
Mean session length (hours) & 0.787 & 1.192 & 0.781 & 0.422 \\
Mean chat sessions & 1.278 & 1.426 & 1.286 & 1.358 \\
Mean hotel searches & 11.33 & 35.772 & 11.245 & 0 \\
Mean clicks & 5.12 & 14.582 & 4.821 & 0 \\
Mean orders & 0.017 & 0.064 & 0.016 & 0.006 \\
Conversion rate (\%) & 1.123 & 1.887 & 1.073 & 0.39 \\
\addlinespace[0.35em]
\multicolumn{5}{l}{\textit{\textbf{Panel C: Chat intent distribution (\%)}}} \\
Attraction & 38.62 & 37.258 & 43.252 & 43.442 \\
Hotel & 33.232 & 43.123 & 29.943 & 8.78 \\
Travel Planning & 6.369 & 3.282 & 4.428 & 8.641 \\
Customer Service & 4.117 & 3.076 & 4.057 & 6.257 \\
Flight & 0.575 & 0.183 & 0.497 & 2.491 \\
Other Transportation & 4.213 & 3.46 & 4.647 & 10.378 \\
Other & 12.874 & 9.616 & 13.176 & 20.012 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\item \textit{Notes}: This table compares four groups of login sessions containing at least one AI chat. The first three groups additionally contain at least one hotel search within the session: \textit{Chat-First} sessions have all chat events before all search events; \textit{Chat-After-Search} have all chat events after all search events; \textit{Chat-Between-Search} have interleaved events. \textit{Chat-Only} sessions contain chat but no hotel search. Panel~A reports the number and share of sessions in each group. Panel~B reports session-level characteristics; differences across the three chat+search groups are all significant at the 0.1\% level (Kruskal--Wallis / chi-squared). Panel~C reports chat intent shares (summing to 100\% per column). Intent differs significantly across the three chat+search groups ($\chi^2 = 1705$, $p < 0.001$). $N = 206,245$ sessions.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Table/Compare_keymetrics_chatuser_nochatuser.tex <==
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\toprule
 & \multicolumn{2}{c}{\shortstack{\textbf{Chat Users}\\ N = 1,904,368}} 
 & \multicolumn{2}{c}{\shortstack{\textbf{Non-Chat Users}\\ N = 29,237,985}} 
 % & \multicolumn{2}{c}{\textbf{Chat Users (N = 1,904,368)}} 
 % & \multicolumn{2}{c}{\textbf{Non-Chat Users (N = 29,237,985)}} 
 &  &  \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Variable} 
& \textbf{Mean} & \textbf{SD}
& \textbf{Mean} & \textbf{SD}
& \textbf{Diff} & \textbf{t-stat} \\
\midrule
female & 0.52 & 0.500 & 0.44 & 0.496 & 0.08 & 204.49 \\
agegroup\_level\_new & 2.62 & 1.096 & 2.19 & 1.180 & 0.43 & 521.85 \\
D\_newuser\_regdate & 0.43 & 0.495 & 0.52 & 0.500 & -0.09 & -230.47 \\
device\_ios & 0.38 & 0.485 & 0.49 & 0.500 & -0.11 & -306.67 \\
vip & 12.92 & 9.614 & 9.34 & 8.649 & 3.58 & 501.29 \\
star & 2.88 & 1.449 & 2.53 & 1.561 & 0.36 & 326.59 \\
localcity\_level & 2.17 & 0.892 & 2.17 & 0.939 & -0.01 & -7.81 \\
N\_query\_total & 150.49 & 619.324 & 66.77 & 347.792 & 83.71 & 184.65 \\
N\_query\_keyword\_total & 44.77 & 246.758 & 19.27 & 122.459 & 25.50 & 141.48 \\
N\_query\_nokeyword\_total & 105.72 & 462.163 & 47.51 & 280.105 & 58.21 & 171.78 \\
N\_query\_star3\_total & 38.70 & 182.373 & 17.49 & 98.388 & 21.21 & 158.98 \\
N\_query\_star4\_total & 37.44 & 170.850 & 15.60 & 84.814 & 21.84 & 174.98 \\
N\_query\_star5\_total & 22.94 & 137.121 & 9.08 & 63.010 & 13.87 & 138.59 \\
N\_unique\_hotel\_total & 71.43 & 183.543 & 34.35 & 112.222 & 37.08 & 275.44 \\
N\_clicks\_total & 66.51 & 184.512 & 28.17 & 89.014 & 38.33 & 284.55 \\
N\_conv\_total & 1.60 & 7.570 & 0.88 & 3.023 & 0.73 & 131.81 \\
N\_order\_amt\_1\_total & 0.25 & 2.900 & 0.17 & 1.348 & 0.08 & 37.10 \\
N\_order\_amt\_2\_total & 0.43 & 2.631 & 0.27 & 1.241 & 0.16 & 84.17 \\
N\_order\_amt\_3\_total & 0.50 & 1.802 & 0.27 & 1.004 & 0.23 & 176.43 \\
N\_order\_amt\_4\_total & 0.19 & 0.735 & 0.09 & 0.449 & 0.10 & 180.14 \\
N\_order\_amt\_5\_total & 0.22 & 0.952 & 0.10 & 0.541 & 0.12 & 170.09 \\
N\_order\_star\_1\_3\_total & 0.90 & 5.387 & 0.54 & 2.293 & 0.36 & 91.37 \\
N\_order\_star\_4\_total & 0.39 & 1.628 & 0.21 & 0.925 & 0.18 & 150.98 \\
N\_order\_star\_5\_total & 0.22 & 1.053 & 0.11 & 0.698 & 0.11 & 141.05 \\
N\_order\_hotel\_total & 1.59 & 6.615 & 0.90 & 2.948 & 0.69 & 142.72 \\
N\_order\_flight\_total & 0.69 & 2.240 & 0.48 & 2.150 & 0.21 & 122.71 \\
N\_order\_train\_total & 1.24 & 3.429 & 0.96 & 2.938 & 0.28 & 110.50 \\
N\_order\_vacation\_total & 0.05 & 0.389 & 0.02 & 0.153 & 0.03 & 110.67 \\
N\_order\_play\_total & 0.04 & 0.923 & 0.01 & 0.372 & 0.03 & 44.69 \\
N\_order\_ticket\_total & 0.41 & 5.288 & 0.12 & 1.597 & 0.29 & 76.58 \\
\bottomrule
\end{tabular}
}
\caption{Descriptive Statistics: Chat vs. Non-Chat Users (Rounded)}
\label{tab:chat_nonchat_summary_rounded}
\end{table}


==> Table/Table_summary_journey_construction.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
Obs. Level & Variable & N & Mean & SD & Min & P25 & Median & P75 & Max \\
\midrule
% Journey & Mean Order Rate & NA & NA & NA & NA & NA & NA & NA & NA \\
% Journey & Avg Gap (Hrs) & NA & NA & NA & NA & NA & NA & NA & NA \\
% Journey & Avg Length (Hrs) & NA & NA & NA & NA & NA & NA & NA & NA \\
Journey & N Clicks & 1{,}535{,}725 & 18.13 & 177.40 & 0.00 & 0.00 & 0.00 & 5.00 & 62{,}211.00 \\
Journey & Length (Hrs) & 25{,}595.42 & 49.28 & 102.31 & 0.00 & 0.23 & 19.54 & 57.92 & 1{,}847.99 \\
Journey & N Orders & 1{,}535{,}725 & 0.44 & 2.44 & 0.00 & 0.00 & 0.00 & 1.00 & 2{,}624.00 \\
% Journey & Total Journeys & NA & NA & NA & NA & NA & NA & NA & NA \\
\midrule
User & Avg Gap (Hrs) & 3{,}143.40 & 102.23 & 101.99 & -2.39 & 45.77 & 71.17 & 118.78 & 1{,}074.81 \\
User & Avg Length (Hrs) & 3{,}143.40 & 10.01 & 44.15 & 0.00 & 2.96 & 6.35 & 10.84 & 1{,}847.99 \\
% User & Clicks & NA & NA & NA & NA & NA & NA & NA & NA \\
% User & Length (Hrs) & NA & NA & NA & NA & NA & NA & NA & NA \\
% User & Orders & NA & NA & NA & NA & NA & NA & NA & NA \\
User & Total Journeys & 188{,}604 & 16.36 & 11.86 & 1.00 & 7.00 & 14.00 & 24.00 & 159.00 \\
\bottomrule
\end{tabular}


==> Table/descriptive_ai_adopt/Chat_adoption_regression_all.tex <==
\begin{table}[H]
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline\\
 % & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
 & \multicolumn{3}{c}{AI Chat Adoption} \\ 
\cline{2-4} 
 & OLS & Logit & Probit\\ 
 & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 iOS Device & $-$0.026$^{***}$ & $-$0.495$^{***}$ & $-$0.240$^{***}$ \\ 
  & (0.0001) & (0.002) & (0.001) \\ 
  VIP 4+ & 0.019$^{***}$ & 0.201$^{***}$ & 0.110$^{***}$ \\ 
  & (0.0002) & (0.003) & (0.001) \\ 
  Star 4+ & $-$0.002$^{***}$ & $-$0.026$^{***}$ & $-$0.014$^{***}$ \\ 
  & (0.0001) & (0.002) & (0.001) \\ 
  Local City: Intl/SAR & $-$0.006$^{***}$ & $-$0.345$^{***}$ & $-$0.168$^{***}$ \\ 
  & (0.0003) & (0.007) & (0.003) \\ 
  Local City: Municipality & 0.002$^{***}$ & 0.013$^{***}$ & 0.008$^{***}$ \\ 
  & (0.0002) & (0.004) & (0.002) \\ 
  Local City: Prov. Capital & $-$0.004$^{***}$ & $-$0.084$^{***}$ & $-$0.040$^{***}$ \\ 
  & (0.0002) & (0.004) & (0.002) \\ 
  Local City: Prefecture City & $-$0.003$^{***}$ & $-$0.055$^{***}$ & $-$0.027$^{***}$ \\ 
  & (0.0002) & (0.004) & (0.002) \\ 
  Female & 0.011$^{***}$ & 0.172$^{***}$ & 0.084$^{***}$ \\ 
  & (0.0001) & (0.002) & (0.001) \\ 
  New User & $-$0.011$^{***}$ & $-$0.220$^{***}$ & $-$0.107$^{***}$ \\ 
  & (0.0001) & (0.002) & (0.001) \\ 
  Age 24- & $-$0.020$^{***}$ & $-$0.264$^{***}$ & $-$0.129$^{***}$ \\ 
  & (0.0002) & (0.004) & (0.002) \\ 
  Age 25-34 & $-$0.022$^{***}$ & $-$0.312$^{***}$ & $-$0.154$^{***}$ \\ 
  & (0.0002) & (0.004) & (0.002) \\ 
  Age 35-49 & $-$0.006$^{***}$ & $-$0.004 & $-$0.006$^{***}$ \\ 
  & (0.0002) & (0.003) & (0.002) \\ 
  Age 50+ & 0.035$^{***}$ & 0.553$^{***}$ & 0.278$^{***}$ \\ 
  & (0.0002) & (0.004) & (0.002) \\ 
  log(1 + Total Queries) & $-$0.017$^{***}$ & $-$0.307$^{***}$ & $-$0.147$^{***}$ \\ 
  & (0.0002) & (0.003) & (0.001) \\ 
  log(1 + Total Clicks) & 0.009$^{***}$ & 0.088$^{***}$ & 0.047$^{***}$ \\ 
  & (0.0001) & (0.001) & (0.001) \\ 
  log(1 + Unique Hotels) & 0.018$^{***}$ & 0.343$^{***}$ & 0.163$^{***}$ \\ 
  & (0.0002) & (0.002) & (0.001) \\ 
  log(1 + Total Hotel Orders) & $-$0.007$^{***}$ & $-$0.142$^{***}$ & $-$0.069$^{***}$ \\ 
  & (0.0001) & (0.001) & (0.001) \\ 
  log(1 + Total Flight Orders) & $-$0.016$^{***}$ & $-$0.259$^{***}$ & $-$0.130$^{***}$ \\ 
  & (0.0001) & (0.002) & (0.001) \\ 
  log(1 + Total Train Orders) & $-$0.009$^{***}$ & $-$0.168$^{***}$ & $-$0.083$^{***}$ \\ 
  & (0.0001) & (0.001) & (0.001) \\ 
  log(1 + Total Vocation Orders) & 0.060$^{***}$ & 0.411$^{***}$ & 0.238$^{***}$ \\ 
  & (0.0004) & (0.005) & (0.003) \\ 
  log(1 + Total Ticket Orders) & 0.057$^{***}$ & 0.409$^{***}$ & 0.234$^{***}$ \\ 
  & (0.0002) & (0.002) & (0.001) \\ 
  log(1 + Total Login Minutes) & 0.009$^{***}$ & 0.346$^{***}$ & 0.148$^{***}$ \\ 
  & (0.0001) & (0.001) & (0.001) \\ 
  log(1 + Tottal Login Sessions) & 0.014$^{***}$ & 0.149$^{***}$ & 0.086$^{***}$ \\ 
  & (0.0001) & (0.002) & (0.001) \\ 
  % Constant & $-$0.011$^{***}$ & $-$4.819$^{***}$ & $-$2.485$^{***}$ \\ 
  % & (0.0003) & (0.006) & (0.003) \\ 
 \hline \\[-1.8ex] 
Observations & 31,129,629 & 31,129,629 & 31,129,629 \\ 
% R$^{2}$ & 0.042 &  &  \\ 
% Adjusted R$^{2}$ & 0.042 &  &  \\ 
% Log Likelihood &  & $-$6,518,038.000 & $-$6,520,466.000 \\ 
% Akaike Inf. Crit. &  & 13,036,124.000 & 13,040,980.000 \\ 
% Residual Std. Error & 0.235 (df = 31129605) &  &  \\ 
% F Statistic & 59,880.110$^{***}$ (df = 23; 31129605) &  &  \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
}
\end{table} 

==> Table/descriptive_ai_adopt/Summary_ask_bu_attribute.tex <==
\begin{table}[H]
\centering
\caption{Share of Attributes in User Requests by User Chat Intents}
\label{tab:intent_final_matrix}

\begin{tabular}{lccccccc}
\toprule
 & & \multicolumn{6}{c}{Share of Different Attributes in User Request (\%)} \\
\cmidrule(lr){3-8}
Chat Intent & Total Share (\%) & Hotel & Person & Place & Price & Time & Transport \\ 
\midrule
Attraction/Travel & 49.46 & 0.57  & 4.84 & 43.51 & 0.98 & 6.18  & 2.43  \\
Hotel             & 17.67 & 29.45 & 2.31 & 45.73 & 2.40 & 1.85  & 1.47  \\
Other             & 22.77 & 0.69  & 2.65 & 24.96 & 0.62 & 2.17  & 11.19 \\
Transportation    & 10.10 & 1.26  & 0.43 & 66.52 & 0.74 & 3.31  & 17.17 \\
% \midrule
% Global Total      & 100.00 & 5.77  & 3.45 & 42.00 & 1.12 & 4.21  & 5.74  \\
\bottomrule
\end{tabular}

\end{table}

==> Table/descriptive_ai_adopt/Summary_userjoruney_10pct_users_wchat.tex <==
% \begin{table}[H]
% \centering
% \caption{Summary Statistics of Chat Usage and User Behavior}
% \label{tab:chat_summary}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccccccccccc}
% \toprule
% \multicolumn{17}{c}{Panel A: Average Journey and Chat Intensity Per User} \\
% \midrule
% Number of Users
% & \multicolumn{2}{c}{Total Journeys}
% & \multicolumn{2}{c}{Hotel Chats}
% & \multicolumn{2}{c}{Activities Chats}
% & \multicolumn{2}{c}{Transport Chats}
% & \multicolumn{8}{c}{} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
% & Mean & SD & Mean & SD & Mean & SD & Mean & SD
% & \multicolumn{8}{c}{} \\
% \midrule
% 18,812
% & 8.502 & 5.230
% & 0.202 & 0.408
% & 0.500 & 0.520
% & 0.101 & 0.308
% & \multicolumn{8}{c}{} \\
% \midrule

% \multicolumn{17}{c}{Panel B: Chat Purpose and Ordering Outcomes} \\
% \midrule
% Chat Purpose
% & \multicolumn{4}{c}{Average Chats (Per Journey)}
% & \multicolumn{4}{c}{Order Probability (\%)}
% & \multicolumn{4}{c}{Average Orders  (Per Journey)}
% & \multicolumn{1}{c}{} \\
% \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
% & Total & Hotel & Transport & Activities
% & Total & Hotel & Transport & Activities
% & Total & Hotel & Transport & Activities
% &  \\
% \midrule
% Activities
% & 1.905 & 0.073 & 1.724 & 0.044
% & 33.66 & 17.80 & 8.26 & 11.45
% & 0.864 & 0.366 & 0.239 & 0.260
% &  \\
% Hotel
% & 1.781 & 1.492 & 0.209 & 0.030
% & 28.70 & 21.97 & 6.49 & 2.39
% & 0.685 & 0.437 & 0.196 & 0.052
% &  \\
% Transport
% & 2.225 & 0.074 & 0.312 & 1.656
% & 25.79 & 8.33 & 17.67 & 2.64
% & 0.895 & 0.266 & 0.539 & 0.090
% &  \\
% \midrule

% \multicolumn{17}{c}{Panel C: User Behavior by Order Status and Chat Purpose} \\
% \midrule
% Chat Purpose
% & \multicolumn{8}{c}{Users With Order}
% & \multicolumn{8}{c}{Users Without Order} \\
% \cmidrule(lr){2-9}\cmidrule(lr){10-17}
% & \multicolumn{2}{c}{Login Time}
% & \multicolumn{2}{c}{Queries}
% & \multicolumn{2}{c}{Clicks}
% & \multicolumn{2}{c}{Keyword Clicks}
% & \multicolumn{2}{c}{Login Time}
% & \multicolumn{2}{c}{Queries}
% & \multicolumn{2}{c}{Clicks}
% & \multicolumn{2}{c}{Keyword Clicks} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
% \cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}
% & Mean & SD & Mean & SD & Mean & SD & Mean & SD
% & Mean & SD & Mean & SD & Mean & SD & Mean & SD \\
% \midrule
% Activities
% & 268.22 & 494.36 & 7.25 & 17.27 & 22.26 & 58.40 & 5.81 & 18.50
% & 258.37 & 1817.66 & 4.96 & 43.41 & 21.86 & 198.21 & 5.43 & 38.45 \\
% Hotel
% & 282.78 & 522.41 & 10.99 & 22.36 & 35.45 & 84.88 & 10.70 & 25.27
% & 402.62 & 2320.81 & 11.24 & 59.80 & 57.51 & 332.56 & 16.31 & 91.23 \\
% Transport
% & 218.45 & 364.38 & 4.58 & 23.04 & 12.29 & 57.96 & 3.50 & 14.36
% & 79.14 & 170.91 & 1.48 & 9.43 & 3.57 & 23.57 & 1.09 & 8.74 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}
\begin{table}[H]
\centering
\caption{Summary Statistics of Chat Usage and User Behavior}
\label{tab:chat_summary}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccc}
\toprule

% =========================
% Panel A
% =========================
\multicolumn{17}{c}{Panel A: Average Journey and Chat Intensity Per User} \\
\midrule
Number of Users
& \multicolumn{2}{c}{Total Journeys}
& \multicolumn{2}{c}{Hotel Chats}
& \multicolumn{2}{c}{Activities Chats}
& \multicolumn{2}{c}{Transport Chats}
& \multicolumn{8}{c}{} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
& Mean & SD & Mean & SD & Mean & SD & Mean & SD
& \multicolumn{8}{c}{} \\
\midrule
18,812
& 8.502 & 5.230
& 0.202 & 0.408
& 0.500 & 0.520
& 0.101 & 0.308
& \multicolumn{8}{c}{} \\
\midrule

% =========================
% Panel B
% =========================
\multicolumn{17}{c}{Panel B: Chat Purpose and Ordering Outcomes} \\
\midrule
Chat Purpose
& \multicolumn{4}{c}{Average Chats (Per Journey)}
& \multicolumn{4}{c}{Order Probability (\%)}
& \multicolumn{4}{c}{Average Orders (Per Journey)}
& \multicolumn{1}{c}{} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
& Total & Hotel & Transport & Activities
& Total & Hotel & Transport & Activities
& Total & Hotel & Transport & Activities
& \\
\midrule
Activities
& 1.905 & 0.073 & 1.724 & 0.044
& 33.66 & 17.80 & 8.26 & 11.45
& 0.864 & 0.366 & 0.239 & 0.260
& \\
Hotel
& 1.781 & 1.492 & 0.209 & 0.030
& 28.70 & 21.97 & 6.49 & 2.39
& 0.685 & 0.437 & 0.196 & 0.052
& \\
Transport
& 2.225 & 0.074 & 0.312 & 1.656
& 25.79 & 8.33 & 17.67 & 2.64
& 0.895 & 0.266 & 0.539 & 0.090
& \\
\midrule

% =========================
% Panel C
% =========================
\multicolumn{17}{c}{Panel C: Journey-Level Summary by Chat Purpose and Order Status} \\
\midrule
Chat Purpose
& \multicolumn{8}{c}{Journey with Order}
& \multicolumn{8}{c}{Journey with No Order} \\
\cmidrule(lr){2-9}\cmidrule(lr){10-17}
& \multicolumn{2}{c}{Total Journeys}
& \multicolumn{2}{c}{Login Time}
& \multicolumn{2}{c}{Total Query}
& \multicolumn{2}{c}{Total Click}
& \multicolumn{2}{c}{Total Journeys}
& \multicolumn{2}{c}{Login Time}
& \multicolumn{2}{c}{Total Query}
& \multicolumn{2}{c}{Total Click} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}
& \multicolumn{2}{c}{N}
& Mean & SD
& Mean & SD
& Mean & SD
& \multicolumn{2}{c}{N}
& Mean & SD
& Mean & SD
& Mean & SD \\
\midrule
Hotel
& \multicolumn{2}{c}{1{,}087}
& 397.08 & 933.86
& 12.75 & 23.60
& 46.59 & 94.85
& \multicolumn{2}{c}{2{,}710}
& 296.81 & 1150.42
& 10.62 & 53.99
& 40.37 & 170.97 \\
Transport
& \multicolumn{2}{c}{520}
& 336.03 & 439.84
& 6.18 & 15.66
& 22.61 & 67.09
& \multicolumn{2}{c}{1{,}480}
& 120.33 & 432.22
& 1.39 & 6.27
& 3.92 & 21.32 \\
Travel/Activities
& \multicolumn{2}{c}{3{,}206}
& 351.84 & 563.26
& 8.33 & 15.71
& 27.24 & 63.37
& \multicolumn{2}{c}{6{,}289}
& 197.41 & 756.44
& 5.00 & 32.32
& 16.81 & 100.06 \\
\bottomrule

\end{tabular}
}
\end{table}


==> Table/descriptive_ai_adopt/Summary_userjoruney_10pct_users_worder.tex <==
\begin{table}[H]
\centering
\caption{Summary of User Journeys}
\label{tab:user_journeys}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccc}
\toprule
\multicolumn{17}{c}{Panel A: Average Journey Per User} \\
\midrule
Number of Users 
& \multicolumn{2}{c}{All Journey}
& \multicolumn{2}{c}{Hotel Journey}
& \multicolumn{2}{c}{Activity Journey}
& \multicolumn{2}{c}{Transportation Journey}
& \multicolumn{8}{c}{} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
& Mean & SD & Mean & SD & Mean & SD & Mean & SD
& \multicolumn{8}{c}{} \\
\midrule
1,571,654
& 10.954 & 5.257
& 1.959 & 7.376
& 0.245 & 0.774
& 1.992 & 3.065
& \multicolumn{8}{c}{} \\
\midrule

\multicolumn{17}{c}{Panel B: Chat Usage by Journey Type} \\
\midrule
Journey Type
& \multicolumn{4}{c}{Chat Usage (\%)}
& \multicolumn{12}{c}{} \\
\cmidrule(lr){2-5}
& Overall & Hotel & Activities & Transportation
& \multicolumn{12}{c}{} \\
\midrule
Activities & 37.83 & 2.57 & 28.05 & 1.66 & \multicolumn{12}{c}{} \\
Hotel & 12.66 & 3.35 & 6.79 & 0.77 & \multicolumn{12}{c}{} \\
Transport & 6.10 & 0.83 & 2.57 & 0.94 & \multicolumn{12}{c}{} \\
\midrule

\multicolumn{17}{c}{Panel C: Chat vs No-Chat User Behavior by Journey Type} \\
\midrule
Journey Type
& \multicolumn{8}{c}{Chat User}
& \multicolumn{8}{c}{No-Chat User} \\
\cmidrule(lr){2-9}\cmidrule(lr){10-17}
& \multicolumn{2}{c}{Total Login Time}
& \multicolumn{2}{c}{Total Queries}
& \multicolumn{2}{c}{Total Clicks}
& \multicolumn{2}{c}{Keyword Clicks}
& \multicolumn{2}{c}{Total Login Time}
& \multicolumn{2}{c}{Total Queries}
& \multicolumn{2}{c}{Total Clicks}
& \multicolumn{2}{c}{Keyword Clicks} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}
& Mean & SD & Mean & SD & Mean & SD & Mean & SD
& Mean & SD & Mean & SD & Mean & SD & Mean & SD \\
\midrule
Activities
& 196.746 & 369.047 & 4.270 & 12.393 & 9.719 & 60.966 & 2.519 & 10.434
& 133.449 & 228.322 & 3.336 & 9.586 & 6.900 & 28.067 & 1.811 & 9.847 \\
Hotel
& 192.259 & 376.259 & 9.139 & 14.864 & 22.273 & 56.837 & 6.434 & 22.618
& 106.327 & 199.054 & 6.664 & 12.414 & 14.089 & 33.975 & 4.059 & 12.691 \\
Transport
& 174.455 & 323.029 & 3.864 & 10.598 & 9.392 & 45.228 & 2.438 & 11.889
& 97.607 & 170.169 & 1.902 & 7.375 & 3.717 & 19.562 & 1.088 & 6.772 \\
\bottomrule
\end{tabular}
}
\end{table}


==> Table/descriptive_ai_adopt/Summary_usersession_how.tex <==
\begin{table}[H]
\centering
\caption{Descriptive Patterns of AI Chat Usage}
\label{tab:ai_usage_patterns}
\begin{small}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
Variable & N & Mean & SD & Min & P25 & Median & P75 & Max \\ 
\hline
\multicolumn{9}{c}{Panel A: Session-Level Interaction (Planning Intensity)} \\
\hline
Queries per Session & 213,460 & 1.31 & 0.94 & 1.00 & 1.00 & 1.00 & 1.00 & 54.00 \\
Session Duration (Min) & 213,460 & 1.81 & 22.13 & 0.00 & 0.00 & 0.00 & 0.28 & 4,062.88 \\
Info Velocity (Chars/Min) & 213,460 & 1,456.52 & 3,710.22 & 1.00 & 642.10 & 1,168.08 & 1,842.50 & 235,620.00 \\
Deep Thinking Enabled (\%) & 213,460 & 0.79 & 0.41 & 0.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
Ever Satisfied (\%) & 213,460 & 0.004 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
\hline
\multicolumn{9}{c}{Panel B: Request-Level Interaction (Information Expansion)} \\
\hline
User Ask Length (Chars) & 280,350 & 10.52 & 13.67 & 1 & 5 & 8 & 12 & 2,501 \\
AI Reply Length (Chars) & 280,350 & 1,089.13 & 717.44 & 1 & 459 & 1,145 & 1,596 & 29,892 \\
User Info Entropy & 280,350 & 1.06 & 0.65 & 0 & 1 & 1 & 1 & 4 \\
AI Info Entropy & 280,350 & 3.07 & 1.78 & 0 & 2 & 4 & 4 & 5 \\
Response Incomplete (\%) & 280,350 & 0.09 & 0.29 & 0 & 0 & 0 & 0 & 1 \\
\hline
\multicolumn{9}{c}{Panel C: Distribution of User Intent (Request-level)} \\
\hline
Category & \multicolumn{3}{c}{Frequency (N)} & \multicolumn{2}{c}{Share (\%)} & \multicolumn{3}{c}{Cumulative (\%)} \\
\hline
Attractions & \multicolumn{3}{c}{118,126} & \multicolumn{2}{c}{42.14} & \multicolumn{3}{c}{42.14} \\
Hotel & \multicolumn{3}{c}{49,547} & \multicolumn{2}{c}{17.67} & \multicolumn{3}{c}{59.81} \\
Other / General & \multicolumn{3}{c}{48,616} & \multicolumn{2}{c}{17.34} & \multicolumn{3}{c}{77.15} \\
Other Transportation & \multicolumn{3}{c}{23,252} & \multicolumn{2}{c}{8.29} & \multicolumn{3}{c}{85.44} \\
Travel Planning & \multicolumn{3}{c}{20,523} & \multicolumn{2}{c}{7.32} & \multicolumn{3}{c}{92.76} \\
Customer Service & \multicolumn{3}{c}{15,214} & \multicolumn{2}{c}{5.43} & \multicolumn{3}{c}{98.19} \\
Flight & \multicolumn{3}{c}{5,072} & \multicolumn{2}{c}{1.81} & \multicolumn{3}{c}{100.00} \\
\hline
\end{tabular}
}
\end{small}
\begin{tablenotes}
\footnotesize
% \item \textit{Notes:} Panel A aggregates interaction data at the session level ($callid$). Panel B presents request-level ($requestid$) summary statistics. Panel C categorizes the primary business intent of each user query. Info Velocity represents the total characters generated per minute of session duration. Entropy measures the structural density of information provided or returned.
\end{tablenotes}
\end{table}
